Reasoning about Moving Target Defense in Attack Modeling Formalisms

Since 2009, Moving Target Defense (MTD) has become a new paradigm of defensive mechanism that frequently changes the state of the target system to confuse the attacker. This frequent change is costly and leads to a trade-off between misleading the attacker and disrupting the quality of service. Optimizing the MTD activation frequency is necessary to develop this defense mechanism when facing realistic, multi-step attack scenarios. Attack modeling formalisms based on DAG are prominently used to specify these scenarios. Our contribution is a new DAG-based formalism for MTDs and its translation into a Price Timed Markov Decision Process to find the best activation frequencies against the attacker's time/cost-optimal strategies. For the first time, MTD activation frequencies are analyzed in a state-of-the-art DAG-based representation. Moreover, this is the first paper that considers the specificity of MTDs in the automatic analysis of attack modeling formalisms. Finally, we present some experimental results using Uppaal Stratego to demonstrate its applicability and relevance.

==> lib/defines.tex <==
\makeatletter
\newcommand{\DeclareLatinAbbrev}[2]{%
  \DeclareRobustCommand{#1}{%
    \@ifnextchar{.}{\textit{#2}}{%
      \@ifnextchar{,}{\textit{#2.}}{%
        \@ifnextchar{!}{\textit{#2.}}{%
          \@ifnextchar{?}{\textit{#2.}}{%
            \@ifnextchar{)}{\textit{#2.}}{%
              {\textit{#2.,\ }}}}}}}}%
}
\makeatother
\makeatletter
\newcommand{\DeclareLatinAbbrevNoComma}[2]{%
  \DeclareRobustCommand{#1}{%
    \@ifnextchar{.}{\textit{#2}}{%
      \@ifnextchar{,}{\textit{#2.}}{%
        \@ifnextchar{!}{\textit{#2.}}{%
          \@ifnextchar{?}{\textit{#2.}}{%
            \@ifnextchar{)}{\textit{#2.}}{%
              {\textit{#2.\ }}}}}}}}%
}
\makeatother
\DeclareLatinAbbrev{\eg}{e.g}
\DeclareLatinAbbrev{\Eg}{E.g}
\DeclareLatinAbbrev{\ie}{i.e}
\DeclareLatinAbbrev{\Ie}{I.e}
\DeclareLatinAbbrev{\etc}{etc}
\DeclareLatinAbbrevNoComma{\etal}{et~al}
\DeclareLatinAbbrev{\cf}{cf}
%\newcommand{\etal}{\textit{et~al.}}

% Theorems
\AtEndEnvironment{proof}{\qed}
\newenvironment{sketchproof} {\begin{proof}[Proof (Sketch)]}{Full proof in the appendix.\end{proof}}

% Parts to compile
\newcommand{\FROMPTA}{}
\newcommand{\FROMPTG}{}
%\newcommand{\ALLPROOFS}{}
%\newcommand{\SHRINK}{}
\newcommand{\LINKSCOLORS}{}

% Shrink related
\newcommand{\shrinkalt}[2]{\ifdefined\SHRINK#1\else#2\fi}
\newcommand{\mysubsection}[1]{\ifdefined\SHRINK\subsubsection{#1.}\else\subsection{#1}\fi}

% FROM PTG PTA...
\newcommand{\fromptaptg}[3]{\ifdefined\FROMPTG\ifdefined\FROMPTA#1\else#2\fi\else#3\fi}

% General commands
\newcommand{\ceil}[1]{{\left \lceil{#1}\right \rceil}}
\newcommand{\floor}[1]{{\left \lfloor{#1}\right \rfloor}}
\newcommand{\brac}[1]{{\left\langle{#1}\right\rangle}}
\newcommand{\probability}[1]{{\mathbb{P}\left[{#1}\right]}}
\newcommand{\dbrac}[2]{{#1}_{#2}}  
\newcommand{\characteristic}[2]{{\mathds{1}_{#2}(#1)}}
\newcommand{\inputproof}[1]{\ifdefined\ALLPROOFS\input{#1}\else\input{#1-short}\fi}


% AMG commands
\newcommand{\AMG}{{\mathcal{T}}}
\newcommand{\AMGgeneral}{\AMG}
\newcommand{\AMGroot}{{g_{0}}}
\newcommand{\Nodes}{\mathbf{N}}
\newcommand{\Edges}{\mathbf{E}}
\newcommand{\Goals}{\mathbf{G}}
\newcommand{\AtomicAttacks}{\mathbf{A}}
\newcommand{\Defenses}{\mathbf{D}}
\newcommand{\reset}{\mathsf{reset}}
\newcommand{\operation}[1]{\diamond_{#1}}
\newcommand{\subTreeg}[2]{\tilde{\zeta}^{#1}({#2})}
\newcommand{\subTreeAMG}[2]{\zeta^{#1}({#2})}
\newcommand{\subTreeDef}[1]{\zeta^{#1}}
\newcommand{\subTree}[2]{\zeta({#2})}
\newcommand{\cost}{c}
\newcommand{\propcost}{c'}
\newcommand{\timefunc}{t}
\newcommand{\proba}{p}
\newcommand{\defended}[2]{\Delta_{#2}}
\newcommand{\defense}[1]{\defended{}{#1}^{-1}}
\newcommand{\children}[2]{\mathsf{Out}_{#1}({#2})}
\newcommand{\Interpret}{I}
\newcommand{\ActivatedSet}{{\mathcal{A}}}
\newcommand{\CompletedSet}{{\mathcal{C}}}
\newcommand{\TriggeredSet}{{\mathcal{D}}}
\newcommand{\AMGDef}{\brac{\Nodes, \Edges, \AMGroot, \operation{}, \Defenses, \cost, \propcost, \timefunc, \proba, \defended{}{}}}

% PTA commands
\newcommand{\PTA}{\mathcal{A}}
\newcommand{\Locations}{L}
\newcommand{\Transitions}{E}
\newcommand{\Clocks}{X}
\newcommand{\Guard}{\mathcal{B}}
\newcommand{\clockReset}{\chi}
\newcommand{\invariants}{\iota}
\newcommand{\loc}{\ell}
\newcommand{\price}{\omega}
\newcommand{\Actions}{\Sigma}
\newcommand{\PTADef}{\brac{\Locations, \loc_0, \Clocks, \Actions, \Transitions, \price, \clockReset, \invariants}}

% PTG commands
\newcommand{\PTG}{\mathcal{G}}
\newcommand{\ControllableActions}{\Actions^c}
\newcommand{\UncontrollableActions}{\Actions^u}
\newcommand{\PTGDefFromScratch}{\brac{\Locations, \loc_0, \Clocks, \ControllableActions, \UncontrollableActions, \Transitions, \price, \clockReset, \invariants}}
\newcommand{\PTGDefFromPTA}{\brac{\PTA, \ControllableActions, \UncontrollableActions}}
\ifdefined\FROMPTA
\newcommand{\PTGDef}{\PTGDefFromPTA}
\else% FROMPTA not defined
\newcommand{\PTGDef}{\PTGDefFromScratch}
\fi% FROMPTA
\newcommand{\OutPTG}{\PTG_\AMG}
\newcommand{\OutPTGDef}{\brac{\Locations_{\AMG}, \loc_{\AMG,0}, \Clocks_\AMG, \UncontrollableActions_\AMG, \ControllableActions_\AMG, \Transitions_\AMG, \price_\AMG, \clockReset_\AMG, \invariants_\AMG}}

% PTMDP commands
\newcommand{\PTMDP}{\mathcal{M}}
\newcommand{\action}{\alpha}
\newcommand{\activate}{\action^\mathsf{act}}
\newcommand{\noactivation}{\bar{\action}^\mathsf{act}}
\newcommand{\completion}{\action^\mathsf{cmp}}
\newcommand{\mtd}{\action^\mathsf{mtd}}
\newcommand{\completionFail}{\bar{\action}^\mathsf{cmp}}
\newcommand{\mtdFail}{\bar{\action}^\mathsf{mtd}}
\newcommand{\strategy}{\mu^c}
\newcommand{\TimeRV}[1]{{T_{#1}}}
\newcommand{\CostRV}[1]{{C_{#1}}}
\newcommand{\PTMDPgoal}{\loc_\AMG}
\newcommand{\density}{\mu^u}
\newcommand{\propagateDefADT}[1]{{\pi^{#1}}}
\newcommand{\propagateDef}[1]{\propagateDefADT{}}
\newcommand{\propagateADT}[2]{{\propagateDefADT{#1}(#2)}}
\newcommand{\propagate}[2]{{\propagateDef{#1}(#2)}}
\newcommand{\pruneDefADT}[1]{{\kappa^{#1}}}
\newcommand{\pruneDef}[1]{{\pruneDefADT{}}}
\newcommand{\pruneADT}[2]{{\pruneDefADT{#1}(#2)}}
\newcommand{\prune}[2]{{\pruneDef{#1}(#2)}}
\newcommand{\fixedPoint}[1]{f_{\propagateDef{#1}}}
\newcommand{\simpleStateADT}[2]{{\lfloor{#2}\rfloor_{#1}}}
\newcommand{\simpleState}[1]{{\simpleStateADT{}{#1}}}
\newcommand{\PTMDPDefFromScratch}{\brac{\Locations, \loc_0, \Clocks, \ControllableActions, \UncontrollableActions, \Transitions, \price, \clockReset, \invariants, \density{}}}
\newcommand{\PTMDPDefFromPTG}{\brac{\PTG, \density{}}}
\newcommand{\runProba}[2]{{\mathbb{P}_{#1, #2}}}
\newcommand{\runExpect}[2]{{\mathbb{E}_{#1, #2}}}
\newcommand{\OutPTMDP}{\PTMDP_\AMG}
\newcommand{\OutPTMDPDefFromScratch}{\brac{\Locations_{\AMG}, \loc_{\AMG,0}, \Clocks_\AMG, \UncontrollableActions_\AMG, \ControllableActions_\AMG, \Transitions_\AMG, \price_\AMG, \clockReset_\AMG, \invariants_\AMG, \density_\AMG{}}}
\newcommand{\OutPTMDPDefFromPTG}{\brac{\OutPTG, \density_\AMG{}}}
\ifdefined\FROMPTG
\newcommand{\PTMDPDef}{\PTMDPDefFromPTG}
\newcommand{\OutPTMDPDef}{\OutPTMDPDefFromPTG}
\else% FROMPTG not defined
\newcommand{\PTMDPDef}{\PTMDPDefFromScratch}
\newcommand{\OutPTMDPDef}{\OutPTMDPDefFromScratch}
\fi% FROMPTG


% OTHER
\newcommand{\coefmu}[2]{{\gamma^{#1}_{(#2)}}}
\newcommand{\diracDef}{\delta}
\newcommand{\dirac}[1]{{\diracDef(#1)}}
\newcommand{\Aof}[1]{{\overline{#1}}}
\newcommand{\Cof}[1]{{\underline{#1}}}
\newcommand{\noDef}{\Nodes_\emptyset}
\newcommand{\delay}{b}
\newcommand{\wait}{\lambda}
\newcommand{\Valuations}{{\mathcal{V}}}
\newcommand{\Delays}{{\mathbb{R}^{+}}}
\newcommand{\CDFPTMDPDef}[2]{{F_{#1,#2}}}
\newcommand{\Strategies}{\mathcal{S}}

% Runs
\newcommand{\RunElements}{T}
\newcommand{\LocVal}{Q}
\newcommand{\cumulativeTimeDef}{T}
\newcommand{\cumulativeCostDef}{C}
\newcommand{\cumulativeTime}[1]{{\cumulativeTimeDef({#1})}}
\newcommand{\cumulativeCost}[1]{{\cumulativeCostDef({#1})}}
\newcommand{\cumulativeTimeGoal}{\hat{\cumulativeTimeDef}}
\newcommand{\cumulativeCostGoal}{\hat{\cumulativeCostDef}}
\newcommand{\Runs}{\mathcal{R}}
\newcommand{\RunsGoal}{\Runs_\AMG}
\newcommand{\nexttc}{\mathsf{acc}}



% OLD
\newcommand{\N}{\mathsf{N}}
\newcommand{\Esp}[1]{\mathbb{E}\left[#1\right]}
\newcommand{\dd}[1]{\mathop{}\!\mathrm{d}#1}


\newcommand{\toremove}[1]{{\color{violet}#1}}
\newcommand{\vad}[1]{\toremove{\color{blue}{Vadim:~#1}}}
\newcommand{\gab}[1]{\toremove{\color{green}{Gab:~#1}}}


% Pre-study
\newcommand{\Prob}[1]{\mathbb{P}\left[#1\right]}
\newcommand\strat[1]{\langle\!\langle#1\rangle\!\rangle}
\newcommand\dstrat[1]{[\![#1]\!]}
\newcommand\nnext{\ocircle}
\newcommand\always{\Box}
\newcommand\eventually{\Diamond}
\newcommand\until{\ \mathcal{U}\ }

==> tex/complexity.tex <==
Size of the AMG $\AMG = \AMGDef$
\begin{align*}
    \vert \AMG \vert &= \Omega((n_a + n_g)^2 + n_d(n_a + n_g))\\
    &= \Omega((n_a +n_g)(n_a+n_g+n_d))
\end{align*}
Size of the PTG $\PTG=\PTGDef$
\begin{align*}
    \vert \PTG \vert &= O(\vert \Locations\vert + n_a\vert \Locations\vert +n_d\vert \Locations\vert)\\
    &= O((n_a +n_d)2^{n_a+n_g})\\
    &= O(2^{\vert \AMG\vert})
\end{align*}

==> tex/semantic.tex <==
An AD-formula over $(\AtomicAttacks, \Defenses)$ is given by the grammar
\begin{align*}
    &S \to \brac{\psi \mid D}\\
    &S \to S \dbrac{\diamond}{D} S\\
    &\psi \to (\psi \diamond \psi)\\
    &\psi \to x_a
\end{align*}
where $S$ is the starting symbol, both $S$ and $\psi$ are non-terminal, $D \subseteq \Defenses$, $\diamond\in \{\land,\lor\}$, $\{\land_D\}_{D \subseteq \Defenses}$ and $\{\lor_D\}_{D \subseteq \Defenses}$ are families of operators, and $(x_a)_{a\in \AtomicAttacks}$ are boolean variables.

Moreover, we say that the AD-formula is \textit{well formed} if for all $a\in \AtomicAttacks$, when $x_a$ appears in $\brac{\psi \mid D}$ where $D \subseteq \Defenses$, then all occurence of $x_a$ in another term $\brac{\psi' \mid D'}$ verifies $D'=D$. \vad{give the intuition of well-formed formula.}

The DAG $t=\brac{\Nodes_{\AMG}, \Edges}$ of an AMG $\AMG = \AMGDef$ can be seen as a term where $\land$ and $\lor$ are \textit{unranked functions}, that is they are a family of function $\land= \{\land^k\}_{k\in \mathbb N}$ and $\lor= \{\lor^k\}_{k\in \mathbb N}$ where for each $k \in \mathbb N$, the function $\lor^k$ and $\land^k$ is $k$-ary. Recursively, any subgoal $g$ with children $n_1, \dots, n_k$ is represented by $\lor^k(n_1, \dots, n_k)$ if $\operation{g} = \lor$, or $\land^k(n_1, \dots, n_k)$ otherwise. This recursion stops when we have only atomic attacks left. Further details and examples are available in~\cite{kordy2010foundations}.

For an AD-signature $\Sigma = \brac{\Goals, \AtomicAttacks, \Defenses, \defense{}{}}$ we define our model $\mathcal M = (M, \Interpret)$ where $M$ is the set of well formed \textit{AD-formulas} over $(\AtomicAttacks, \Defenses)$ and $\Interpret$ is defined recursively as follows.
\begin{itemize}
    \item $\Interpret(a) = \brac{x_a \mid \defense{a}}$ for $a \in \AtomicAttacks$, where $x_a$ is a boolean variable,
    \item for $g \in \Goals$, $\diamond = \operation{g}$, and $g= \diamond^k(n_1, \dots, n_k)$,
    \begin{align*}
        \Interpret(\diamond^k(n_1, \dots, n_k)) =
        \left(\Interpret(n_1) \dbrac{\diamond}{\defense{g}} \dots \dbrac{\diamond}{\defense{g}} \Interpret(n_k)\right)
    \end{align*}
\end{itemize}

We explain the semantic of the model with the following equations where $\psi, \psi_1, \psi_2$ are predicates formulas, $X, X_1, X_2, X_3, X_4, Y, Z$ are well formed AD-formulas, $\diamond \in \{\land, \lor\}$ is a refinement (where $\bar{\land} = \lor$ and $\bar{\lor} = \land$), and $D, D_1, D_2$ are subsets of $\Defenses$.
\begin{itemize}
    \item $(\brac{\psi_1 \mid D}\dbrac{\diamond}{D}\brac{\psi_2\mid D}) = \brac{((\psi_1)\diamond(\psi_2))\mid D}$ (left linearity)
    \item $X \dbrac{\diamond}{D} Y = Y \dbrac{\diamond}{D} X$ (commutativity)
    \item $X \dbrac{\diamond}{D} (Y \dbrac{\bar\diamond}{D} Z) = (X \dbrac{\bar\diamond}{D} Y) \dbrac{\diamond}{D} (X \dbrac{\bar\diamond}{D} Z)$ (distributivity)
    \item $X \dbrac{\diamond}{D} (Y \dbrac{\diamond}{D} Z) = (X \dbrac{\diamond}{D} Y) \dbrac{\diamond}{D} Z$ (associativity)
    \item $X \dbrac{\lor}{\emptyset} (Y \dbrac{\diamond}{D} Z) = X \dbrac{\lor}{\emptyset} (Y \dbrac{\diamond}{\emptyset} Z)$ ($\lor$-absorption) %\gab{petit nom perso... Est-ce que ca sert?})
    \item $(X_1 \dbrac{\diamond}{\emptyset} X_2) \dbrac{\land}{D} (X_3 \dbrac{\diamond}{\emptyset} X_4) = (X_1 \dbrac{\diamond}{\emptyset} X_2)  \dbrac{\land}{\emptyset} (X_3 \dbrac{\diamond}{\emptyset} X_4))$ (no defense absorption)
    \item the normal predicates transformations are possible on $\psi$ in $\brac{\psi \mid D}$ if they don't make negation appear. \vad{How can you use negation? It is not included in your syntax. Are the predicate formulas $\psi, \psi_1, \psi_2$ the same described in your syntax?}
\end{itemize}

The semantic of the AMG is defined by the equivalence relation $\AMG_1 \sim_\mathcal{M} \AMG_2$ if the DAG $t_1$ and $t_2$ of $\AMG_1$ and $\AMG_2$ verify $\Interpret(t_1) = \Interpret(t_2)$ \gab{(ajouter que $\omega, p, t$ doivent être les memes)}. \vad{It is not clear how you can extend $\Interpret$ to handle structures instead of single nodes.}

Given a well formed AD-formula $\psi$, it is possible to obtain a DAG for AMG. For each $x_a$, with $a\in \AtomicAttacks$, we know there is a unique $D \subseteq \Defenses$ such that $x_a$ appears in $\brac{\psi'\mid D}$. We set $\defense{a} = D$. Then we create a subgoal for every $\psi_1 \diamond \psi_2$ and ... \gab{C'est long à décrire et assez intuitif, est-ce que je m'embête pour rien ?} \vad{It could be useful for the reader.}

\textbf{Draft correctness of the semantics:} We want to prove that two AMG $t_1, t_2$ \vad{you use different symbols for the AMG and $t_1, t_2$ are used for the time} that are equivalent ($\Interpret(t_1) = \Interpret(t_2)$) have the same $F_t: t\mapsto \Prob{T\leq t \land \AMGroot \text{ reached }}$ and $F_c: c\mapsto \Prob{C\leq c \land \AMGroot \text{ reached }}$ where $T$ is the random variable of the time, and $C$ is the random variable of the cost in the PTMDP, for some strategy for the attacker. For that we just need to show that the transformation on AD-formulas keep the $F_t$ and $F_c$. \vad{what is the meaning of the latter functions?}
\begin{itemize}
    \item the linearity, commutativity, $\lor$-absorption, and no defense absorption do not change the PTMDP $\to$ OK without change in the strategy
    \item distributivity: TODO
    \item associativity: TODO
    \item $\psi$ transformation: TODO
\end{itemize}

\gab{Est-ce que le reste de la section sert ?} \vad{I think it is very important to well understand the framework. However, I'm not sure this is the right point to intruduce these aspects.} 



==> tex/state-of-the-art.tex <==
\section{Introduction}

Moving Target Defense is an encouraging defense mechanism for system security that get increasing interest from the computer science community since its conception in 2009. However, this research matter is not mature yet and lacks configuration study. Moreover, game theory can formalize situations where different agents have conflicting goals and want to make optimal decisions. Thus, the game-theoretical approach is a classical viewpoint for providing a mathematical framework for cybersecurity. As the security specifications and the attack scenarios can be complex, we can use the power of model-checking and its extension to multi-agent system verification.

This master thesis aims at proposing a method to determine the optimal configuration of Moving Target Defenses through game theory and multi-agent model checking. This Pre-study will present the state of the art of Moving Target Defenses in Section~\ref{sec:mtd}. Section~\ref{sec:game} will introduce basic concepts of game theories and more advanced game representations and classical games. Finally, Section~\ref{sec:sys-verif} will deal with multi-agent system verification by presenting model-checking and its multi-agent adaptation for modeling and system specification.

\section{Moving Target Defense (MTD)}\label{sec:mtd}

\subsection{Motivation for MTDs}

Traditional defense mechanisms are primarily \textit{static} or \textit{reactive}. For example, a firewall that rejects all messages from IP addresses of the form 167.250.000.000/24 is \textit{static}, and an antivirus that scans a program's signature to compare it with a malware signature database and abort the program in case of matching is \textit{reactive}.

On the contrary, MTD mechanisms tend to be \textit{proactive}, that is, they take action before detecting any suspicious activity. Proactivity has two significant implications: one the one hand, the security against \textit{zero-day attacks} (unknown attacks) or \textit{evasive attacks} (meaning the attacker find ways to hide his activity) may be considerably strengthened; on the other hand, they can be activated even when there are no attacks, implying unnecessary cost. This raises the importance of developing a good activation strategy for MTD mechanisms.

Proposed for the first time as a defense paradigm in 2009~\cite{ghosh2009moving}, MTD is yet to become a mature research field. However, some commercial implementations already exist\footnote{\url{https://polyverse.com/}, \url{https://www.morphisec.com/}, \url{https://www.trapx.com}, and \url{https://www.peratonlabs.com/cybervan.html}}. The scientific community's interest in MTD holds as shows the increasing number of new proposals in MTDs for IoT. It raised from 3 or 4 proposals a year between 2013 and 2015 to a range of 5 to 8 proposals a year between 2016 and 2019~\cite{navas2020mtd}.

\subsection{What is MTD?}

MTD is a defense technique where the \textit{state} of the target system \textit{moves} frequently. The \textit{state} of the system is its configuration (e.g. IP address of a server, Operating system used, version of a library, passwords of some users...). Later, it will be referred to as the \textit{moving parameter} (MP) of the MTD mechanism. To \textit{move} the MP corresponds to changing its value, how to do it and when are essential questions of MTD design.

The typical structure of an attack (e.g. categorized in the \textit{cyber-kill-chain}\footnote{\url{https://www.lockheedmartin.com/en-us/capabilities/cyber/cyber-kill-chain.html}}) always starts with probing the system to understand its configuration and plan vulnerability exploitation. With the MTD mechanism, the attacker cannot spend unlimited time to find a vulnerability in a single state of the target, as this state will change frequently.

\subsection{Objective of MTD}

The main objective of Moving Target Defense is to break the asymmetry between the attacker and the defender. In a classical attack/defense scheme, the attacker would automatically probe the system with tools like \verb+nmap+ to detect, say, open ports and running services and their version. Then the attacker could search for any known vulnerabilities for the specific versions of the services to plan an attack. In this setting, an MTD defense could, for instance, regularly swap the mapping between the ports and the services to confuse the attacker. The MTD defenses will invalidate the knowledge acquired by the attacker during its reconnaissance phase.

\subsection{Advantages of MTD}

MTDs are meant to increase the complexity, uncertainty, and unpredictability of the system for the attacker. This is known as \textit{security hardening} and is efficient for slowing down implementations of zero-day attacks that is a significant challenge as about one zero-day attack is discovered every week (Figure~\ref{fig:0-day}). Furthermore, The MTD defense is not meant to replace traditional defense methods but is complementary to them to add an extra layer of confusion for the attacker.

\begin{figure}[H]
    \centering
    \includegraphics[width=0.9\columnwidth]{figures/0-day.png}
    \caption[Zero-day vulnerabilities discovered per year]{Zero-day vulnerabilities discovered per year\footnotemark}
    \label{fig:0-day}
\end{figure}
\footnotetext{\url{https://www.zero-day.cz/database/}}

\subsection{MTD Design}

To have a well-defined MTD mechanism, three characteristics must be defined:
\begin{enumerate}
    \item WHAT: specifying the moving parameter, i.e. the configuration of the system that will move,
    \item HOW: the set of valid states for the MP and the decision method for the next state,
    \item WHEN: decide when to change the configuration.
\end{enumerate}
This common terminology is advocated in several surveys about MTD~\cite{sengupta2020survey,navas2020mtd}.


\subsubsection{WHAT}


\renewcommand{\arraystretch}{1.5}
\begin{table*}[t]
    \centering
    \begin{tabular}{|c|c|c|}
    \hline
      \textbf{Layer} & \textbf{Possible} MP & \textbf{Example}\\
      \hline\hline
      \textbf{Data} & format, encoding, representation &
      Dynamic key-Length-Based Security Framework~\cite{puthal2015dynamic}\\
      \hline
      \textbf{Software} & binary,
      application & Dynamic
      Application Rotation Environment~\cite{thompson2016dynamic}\\
      \hline
      \textbf{Runtime env.} & RAM addresses, instruction
      set & Address Space Layout Randomization (ASLR)\\
      \hline
      \textbf{Platform} & CPU architecture, OS, VM &
      Multiple OS Rotational Environment (MORE)~\cite{thompson2014multiple}\\
      \hline
      \textbf{Network} & protocol, topology, IP address &
      Stream Splitting~\cite{evans2019stream}\\
      \hline
    \end{tabular}
    \caption{System layer's classification for the moving parameter.}
    \label{tab:mp-layers}
\end{table*}
\renewcommand{\arraystretch}{1}

The moving parameter of the system can generally fit in one of the five system layers, as described in Table~\ref{tab:mp-layers}. The \textit{data layer} includes the representation of the sensitive data. It can be the storage representation (format) or the representation during the transmission (encoding). An example of such an MTD defense mechanism is the Dynamic key-Length-Based Security Framework~\cite{puthal2015dynamic}. In this framework, the protagonists of a communication agree on a local synchronized key generator to change the encryption regularly without requiring extra communication. This reduces the quantity of cyphertext an attacker can intercept for a given key.

The second layer is the \textit{software layer}. It includes changing the version of the same software or altering the binary code of the identical program. A textbook example is the Dynamic Application Rotation Environment~\cite{thompson2016dynamic}. In this framework, a web interface can have two web servers (Nginx and Apache) that take over each other after a while, making the attacker confused about the attack's target web server.

The third layer is the \textit{runtime environment}. Mechanisms in this category typically change the memory management like the well spread Address Space Layout Randomization (ASLR). This mechanism is implemented by default on Linux, Windows, and Mac OS. It randomizes the position of the memory sections (like \textit{text, stack, heap}) in order to prevent the exploit of memory attacks like buffer overflows.

The fourth layer is the \textit{platform}. This includes OS change, VM change, or even hardware like CPU change. We can cite the Multiple OS Rotational Environment as an example~\cite{thompson2014multiple}. In this mechanism, the active OS is taken periodically from a queue of safe OSs. After the rotation, the old OS is scanned to detect any anomaly and put back on the queue or deleted. Even if the attacker manages to infect an OS, he may not harm the system because the OS is put in quarantine and a new one is activated.

\begin{figure}[H]
    \centering
    \includegraphics[width=0.7\textwidth]{figures/IoT layers.png}
    \caption{Taxonomy distribution of MTD techniques for IoT~\cite{navas2020mtd}.}
    \label{fig:iot-layers}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=0.9\textwidth]{figures/GP layers.png}
    \caption{Taxonomy distribution of general MTD techniques~\cite{navas2020mtd}.}
    \label{fig:gp-layers}
\end{figure}

Finally, the last layer is the \textit{network layer}. A great variety of proposals in this layer exists for IoT (Figure~\ref{fig:iot-layers}). Possible moving parameters are the topology of the network, the protocols used, or the IP address and ports. An industrial example is Stream Splitting~\cite{evans2019stream}, where the payload of a TCP transmission is split on several flows taking different routes. If a router is infected, the attacker has access to only part of the sensitive data.



In Figure~\ref{fig:gp-layers}, we can see the distribution of new MTD proposals (from a survey of 89 papers) among the system layers. Figure~\ref{fig:iot-layers} presents the distribution restricted to IoT proposals. We can notice the prominence of network-level proposals, probably due to the lower implementation cost for embedded systems, while the platform layer only counts one proposal among the 39 surveyed.



\subsubsection{HOW}

The "how" addresses two questions. Firstly, defining the set of valid states for the moving parameter. Secondly, defining the transition function of one state to the next one. Intuitively, a more extensive set of possible states induces more security as the attacker cannot brute-force all the states to continue his attack whatever the current state. Nevertheless, the "HOW" should also guaranty the unpredictability of the MP. Thus the size of the state set is not the only point that matters. The transition function should be well designed, such that the choice of the following state is not predictable.

The unpredictability for a random variable $X$ is often measured with the entropy $H(X)$.
\begin{equation*}
    H(X) = - \sum_{x\in X(\Omega)} \Prob{X=x}\log\left(\Prob{X=x}\right)
\end{equation*}

Higher entropy means more unpredictability and is desired for the moving parameter. It can be shown that the entropy is maximal for a uniform distribution. Nevertheless, it is not necessarily the optimal transition function because two states in a row should expose an \textit{attack surface} (intuitively the set of channels, methods, and data items that an attacker could use for an intrusion~\cite{manadhata2010attack}) as different as possible. If two states in a row have the same vulnerability, the attacker can exploit the vulnerability during the two states' exposure time.

The sets of states for the MP can be obvious (e.g. set of the available IP address). If not, there are two techniques to generate states: \textit{diversification} and \textit{redundancy}. \textit{Diversification} means using a different object with the same functionality, for example, semantically identical programs with different implementations. Program diversity can be achieved through compiler diversification. Another method could be to insert \verb+NOP+ (no-operation) randomly within the binary of executables. \textit{Redundancy} means that several same components are used to achieve the function. For example, a system could unpredictably use many hardware RAMs to confuse the attacker using a side-channel memory attack. Similarly, the network traffic could travel through different paths to avoid a centralized attack on a single node as in Stream Splitting~\cite{evans2019stream}.

The most used transition function is randomization, which is choosing the next state independently with uniform distribution in the set of available states. This leads to optimal entropy as the unpredictability is maximal.

\subsubsection{WHEN}

Less studied, the question of "WHEN" is, however, essential. The reconfiguration can cost many resources and disrupt the quality of service, but it should happen often enough, so the attacker's knowledge about the system is invalidated between the probing and the actual attack. There is a trade-off that needs to be addressed here, and that is one goal of my research project.

We distinguish mainly three methods to determine when to change states. The first one is \textit{time-based}: the system is reconfigured proactively after a fixed period of time. For example, IP address randomization, which is discussed by many proposals~\cite{antonatos2007defending,dunlop2011mt6d,clark2013effectiveness}, could be triggered every 5 minutes. The second method is \textit{event-based}. In this case, the movement happens either reactively (when detecting a suspicious activity) or on a non-time-based event (like the reception of every megabyte of data).


\subsection{Challenges of MTD}

\subsubsection{Costs}

There are three sources of costs in MTDs. The first is the cost of \textit{generating} a state. The second is the cost of state \textit{storage}, and the third is the cost of state \textit{migration}. The value of these costs highly depends on the actual MTD mechanism. In the example of port shuffling evoked earlier, the state generation requires a pseudo-random number generator to obtain the new mapping. Then the storage is just an array of integers, and finally, the migration cost would depend on how each service interruption is handled.

\subsubsection{State Design}

The choice of the moving parameter and the state space is a significant challenge. Firstly, the state space must be large enough so that the attacker cannot easily prepare an attack for each state. If there are only two configurations, the attacker can prepare two attack scenarios.

Secondly, two configurations in a row should, ideally, have an empty intersection of their attack surface. In the example of the port shuffling, if two states in a row have a service that is not remapped, an attack on this service can be carried on for a longer time.

\subsubsection{Activation Frequency}

This subsection deals with time-based MTDs, that is, MTD with a fixed activation frequency. If the activation frequency is high, on the one hand, the attacker has less time to plan his attack, but on the other hand, the Quality of Service (QoS) could be disrupted due to the resource consumption of the migration and the discontinuity of the service. This trade-off between QoS and the effectiveness of time-based MTD has not been addressed enough in the literature, even though it is a crucial point of MTD applicability in real life. As a result, This challenge requires an optimal timing strategy for the MTD activation frequency that considers the costs, the QoS, and the threat characteristics (like the expected time of a specific attack).

\section{Game Theory}\label{sec:game}

Many papers address security questions from the viewpoint of game theory. The attacker and defender are two agents in a conflicting situation aiming to make optimal decisions. This is precisely what formalizes the game theory mathematically, and it gives the notion of value to the game, optimal strategy, equilibrium... There are different representations for a game that we will highlight in the following subsection.

\subsection{Game Representation}

\subsubsection{Normal Form}

The normal form represents a two-player game with a different payoff per player or zero-sum (the payoff of one player is the opposite of the payoff of the other). A famous example is the prisoner dilemma (Table\ref{tab:prisoner-nf}): two prisoners, $P_1$ and $P_2$, are isolated in two rooms and are given two options independently. Either they betray the other (strategy $B$) or stay silent (strategy $S$). If both betray the other, they take two years of prison each. If both stay silent, they will undergo one year of prison each. If one betrays the other that stays silent, the traitor gets no prison, and the other goes three years to jail. In the modeling, the payoff is the incarceration year's opposite so that each prisoner wants to maximize its payoff.

\begin{table}[H]
    \centering
    \begin{tabular}{c|c|c}
         & $P_1\to B$ & $P_1\to S$  \\
         \hline
        $P_2\to B$ & $-2,-2$ & $-3,0$ \\
        \hline
        $P_2\to S$ & $0,-3$ & $-1,-1$
    \end{tabular}
    \caption{Normal form of the prisoner dilemma. Each prisoner $P_1$ and $P_2$ can betray the other ($B$) or stay silent ($S$). A payoff $(-a,-b)$ means that $P_1$ will spend $a$ year in prison, and $P_2$ will spend $b$ years in prison.}
    \label{tab:prisoner-nf}
\end{table}

\subsubsection{Extensive Form}


\begin{figure}[H]
    \centering
    \subfloat[\centering]{
    \begin{tikzpicture}[
        sibling distance=7em,
        level distance=7em,
        every node/.style = {{font=\footnotesize}},
        edge from parent/.style = {draw, -latex},
        sloped]
      \node [root] {Init}
        child {
            node [rtreenode] {$-2,-2$}
            edge from parent node [above] {$P_1\to B$}
            edge from parent node [below] {$P_2\to B$}
        }
        child {
            node [rtreenode] {$0,-3$}
            edge from parent node [above] {$P_1\to B$}
            edge from parent node [below] {$P_2\to S$}
        }
        child {
            node [rtreenode] {$-3,0$}
            edge from parent node [above] {$P_1\to S$}
            edge from parent node [below] {$P_2\to B$}
        }
        child {
            node [rtreenode] {$-1,-1$}
            edge from parent node [above] {$P_1\to S$}
            edge from parent node [below] {$P_2\to S$}
        };
    \end{tikzpicture}
    \label{fig:concurrent}
    }
    
    \subfloat[\centering]{
    \begin{tikzpicture}[
        level 1/.style = {level distance=3em, sibling distance=14em},
        level 2/.style = {level distance=5em, sibling distance=7em},
        every node/.style = {{font=\footnotesize}},
        edge from parent/.style = {draw, -latex},
        sloped]
      \node [root] {Init}
        child {
            node [treenode] {$B$}
            child {
                node [rtreenode] {$-2,-2$}
                edge from parent node [above] {$P_2\to B$}
            }
            child {
                node [rtreenode] {$0,-3$}
                edge from parent node [above] {$P_2\to S$}
            }
            edge from parent node [above] {$P_1\to B$}
        }
        child {
            node [treenode] {$S$}
            child {
                node [rtreenode] {$-3,0$}
                edge from parent node [above] {$P_2\to B$}
            }
            child {
                node [rtreenode] {$-1,-1$}
                edge from parent node [above] {$P_2\to S$}
            }
            edge from parent node [above] {$P_1\to S$}
        };
    \end{tikzpicture}
    \label{fig:turn}
    }
    
    \subfloat[\centering]{
    \begin{tikzpicture}[
        level 1/.style = {level distance=3em, sibling distance=14em},
        level 2/.style = {level distance=5em, sibling distance=7em},
        every node/.style = {{font=\footnotesize}},
        edge from parent/.style = {draw, -latex},
        sloped]
      \node [root] {Init}
        child {
            node [treenode] (B) {$B$}
            child {
                node [rtreenode] {$-2,-2$}
                edge from parent node [above] {$P_2\to B$}
            }
            child {
                node [rtreenode] {$0,-3$}
                edge from parent node [above] {$P_2\to S$}
            }
            edge from parent node [above] {$P_1\to B$}
        }
        child {
            node [treenode] (S) {$S$}
            child {
                node [rtreenode] {$-3,0$}
                edge from parent node [above] {$P_2\to B$}
            }
            child {
                node [rtreenode] {$-1,-1$}
                edge from parent node [above] {$P_2\to S$}
            }
            edge from parent node [above] {$P_1\to S$}
        };
    \draw[dashed] (B) -- (S);
    \end{tikzpicture}
    \label{fig:inf-set}
    }
    \caption{Three versions of the prisoner dilemma in extensive form. In~\protect\subref{fig:concurrent}, both prisoners have to choose their actions concurrently, while in~\protect\subref{fig:turn}, $P_2$ has access to the decision of the $P_1$ before deciding. The game~\protect\subref{fig:inf-set} with two nodes in the information set means that $P_2$ does not know if the game is in the state $B$ or $S$. As a result, it is equivalent to the game~\protect\subref{fig:concurrent}.}
    \label{fig:prisoner-ext}
\end{figure}

In extensive form, more than two agents can intuitively be represented. Moreover, the sequence of actions is also depicted. The game is represented as a tree where the edges are labeled with each player's combination of actions. The difference between concurrent games and turn-based games can easily be represented in extensive form as in Figure~\ref{fig:prisoner-ext}. The payoff is indicated in the tree's leaves, and a path in the tree is a possible scenario.

In the extensive form, we can also add \textit{information sets} that describe the fact that an agent does not have complete information about the state of the game. If several states are in an information set, the next player does not know the state of the game among the ones of the information set.



\subsection{Strategies}

A strategy is a decision function. There are different types of strategies according to how much memory they have. A memory-less strategy $f_{\neg\text{mem}}$ tells the player what action to choose from a given state of the game. In chess, a memory-less strategy would give the next move according to a snapshot of the board.
$$\forall s\in S, f_{\neg\text{mem}}(s) \in A_s$$

A strategy with full memory $f_\text{mem}$ gives the next move for each possible game history. In chess, it could give different moves for two different histories that led to the same position of pieces on the chessboard. One could intuit that memory is not required in chess to play optimally because the sequences of actions that led to a state will not change anything in the outcome.
$$\forall s\in S, \forall \pi \in \mathcal C(S,s), f_\text{mem}(\pi) \in A_s$$
where $\mathcal C(S,s)$ is the set of valid (i.e. that transition between states follow edges) histories that end in state $s$.


Finally, there can be strategies with finite memory $f_{w\text{-mem}}$ that have access to a finite number $\omega$ of previous states.

Formally, for a game $\mathcal G$ with states set $S$ and player's actions $A_s$ in a state $s\in S$, a strategy takes a valid history of the game as input, that is, a history where the transitions between states follow edges. Let $\mathcal H(\mathcal G,\pi)$ the set of valid histories finishing with the valid sequence of states $\pi\in S^+$. A strategy is a function such that for all $s\in S$ and $\pi \in \mathcal H(\mathcal G,s)$, $f(\pi) \in A_s$. We have the properties,
\begin{align*}
    &\forall s\in S, \forall (\pi, \pi') \in \mathcal H(\mathcal G,s)^2, f_{\neg\text{mem}}(\pi) = f_{\neg\text{mem}}(\pi')\\
    &\forall \pi_\omega\in S^{\omega}, \forall (\pi, \pi') \in \mathcal H(\mathcal G,\omega)^2, f_{\omega\text{-mem}}(\pi) = f_{\omega\text{-mem}}(\pi')\\
\end{align*}

All the strategies described before are called \textit{pure} strategies because they output a decision that is an action for the player. Nevertheless, in games like rock-paper-scissor, the pure strategies do not reflect the intuition since non of "playing rock", "playing paper" or "playing scissors" is a good strategy if the other player guesses our strategy. This case is best modeled with \textit{mixed} strategies, where, for a history $\pi$ finishing in state $s$, the decision is a probability measure of $A_s$ assigning the probability of taking each action. The intuitive "good" strategy in rock-paper-scissor is to do rock, paper, or scissors with a probability of $1/3$ each. This is a mixed strategy.

\subsection{Nash Equilibrium}

A fundamental notion of game theory is the Nash equilibrium. It is the situation in which changing one player's strategy unilaterally will not increase his payoff. In the prisoner dilemma (Table~\ref{tab:prisoner-nf}), the Nash equilibrium is $(P_1\to B, P_2\to B)$. Indeed, in any situation where a player is not betraying, he could increase his payoff by betraying the other (from $-1$ to $0$ if the other is silent, from $-3$ to $-2$ if the other betrays). This leads to the paradoxical outcome: each prisoner goes two years to prison and could only do one year if they both stayed silent. This paradox comes from the hypothesis that every agent considers that the other agent is rational, that is, will want to maximize his payoff.

\subsection{Games on Concurrent Graph Structures}



A graph structure $\mathcal G=\brac{V,E}$ with vertices $V$ and edges $E$ can be the playground for a game. Players' actions from a vertex $v\in V$ lead to the choice of an edge $e\in E$ from $v$ to a new state of the game. The player must then choose new actions to continue the game's progress. The graph can be augmented with weights and clocks, leading to a quantitative or timed game. The vertices are often labeled with boolean properties that can be used to define the rule of the game. The game is turn-based if a player is associated with each vertex and chooses unilaterally the next edge to follow (for example in Figure~\ref{fig:graph}). For non-quantitative games, the solution is, for each node, whether there is a winning strategy starting the game from this node. For quantitative games, we are often interested in the minimum payoff the maximizer player can guaranty himself.

The rest of this section presents some typical examples of games on graph structures.



\begin{figure}[H]
    \centering
    \begin{tikzpicture}[
            ->,
            >=stealth',
            shorten >=1pt,
            auto,
            node distance=2.8cm,
            semithick
        ]

      \node[p1node] (A)                    {$q_a$};
      \node[p2node] (B) [above left of=A] {$q_b$};
      \node[p2node] (D) [above right of=A] {$q_d$};
      \node[p1node] (C) [above right of=B] {$q_c$};
      \node[p2node] (E) [right of=D]       {$q_e$};
    
      \path (A) edge              node {L} (B)
                edge              node {R} (C)
            (B) edge [loop above] node {L} (B)
                edge              node {R} (C)
            (C) edge              node {L} (D)
                edge [bend left]  node {R} (E)
            (D) edge [loop below] node {R} (D)
                edge              node {L} (A)
            (E) edge [bend left]  node {R,L} (A);
    \end{tikzpicture}
    \caption{Example of a two-player turn-based graph structure. Lozenge states belong to the first player, and round states belong to the second player. They both have the possible actions R and L.}
    \label{fig:graph}
\end{figure}


\subsubsection{Reachability Games}

The reachability objective in a two-player game on graph structure $\mathcal G=\brac{ V,E}$ is given by a set of vertices $R\subseteq V$. The first player needs to force the game to enter that state, and the second player must prevent it (Figure~\ref{fig:graph-reach}). We can find variants of this game in the literature: on infinite graphs, on turn-based structures, with deterministic strategies, or mixed ones. The reachability objective is solved \textsf{PTIME} and, for example, deterministic strategies on concurrent finite graphs can be found in linear time~\cite{de2007concurrent}.


\begin{figure}[H]
    \centering
    \begin{tikzpicture}[
            ->,
            >=stealth',
            shorten >=1pt,
            auto,
            node distance=2.8cm,
            semithick
        ]

      \node[p1node] (A)                    {$q_a$};
      \node[p2node] (B) [above left of=A] {$q_b$};
      \node[p2node] (D) [above right of=A] {$q_d$};
      \node[p1node] (C) [above right of=B] {$q_c$};
      \node[p2node, bottom color=yellow!30] (E) [right of=D]       {$q_e$};
    
      \path (A) edge              node {L} (B)
                edge [very thick] node {\textbf{R}} (C)
            (B) edge [loop above] node {L} (B)
                edge              node {R} (C)
            (C) edge              node {L} (D)
                edge [very thick, bend left]  node {\textbf{R}} (E)
            (D) edge [loop below] node {R} (D)
                edge              node {L} (A)
            (E) edge [very thick, bend left]  node {R,L} (A);
    \end{tikzpicture}
    \caption{In this turn-based two-player game, lozenge states belong to the first player, and round states belong to the second player. The first player has reachability objective $\{q_c\}$. Player one has a winning strategy only from the nodes $q_a$, $q_c$, and $q_e$, always choosing the action $R$.}
    \label{fig:graph-reach}
\end{figure}

\subsubsection{Büchi Games}

Büchi games are two-player turn-based games on graph structure $\mathcal G=\brac{ V,E}$. A play is an infinite sequence of moves $\pi\in V^*$. The first player wins if the \textit{acceptance condition} is met for the vertices occurring infinitely often in $\pi$ noted $\bar{\pi} \subseteq V$. The Büchi acceptance condition is given by a set $R\subseteq V$ of nodes. The play $\pi$ is accepted if $\bar{\pi}\cap R\neq \emptyset$.

Büchi games are \textsf{PTIME} and can be solved in $O(n\cdot m)$ for $n=\vert V\vert$ and $m=\vert E\vert$, under some conditions on the outdegrees $\delta(n)$ for instance, the Büchi game can be solved in $O(nm\frac{\log\delta(n)}{\log n})$ as in~\cite{chatterjee2008algorithms}.

\subsubsection{Rabin and Streett Games}

Rabin and Streett games are played on two-player turn-based graph structures with a more elaborated acceptance condition than Büchi games. The Rabin acceptance condition $\{\brac{G_1, R_1}, \dots, \brac{G_k, R_k}\}$ where the $G_i$ and $R_i$ are subsets of $V$ is the following. The play $\pi$ is accepted if there exists $i\in \{1, \dots, k\}$ such that $\bar{\pi}\cap G_i\neq \emptyset \land \bar{\pi}\cup R_i= \emptyset$. The acceptance condition for the Streett game is the dual of the Rabin's one, that is, $\bar{\pi}\cap G_i= \emptyset \lor \bar{\pi}\cup R_i\neq \emptyset$.

There are algorithms to find the winning strategy if it exists for Rabin and Streett games. Some examples run in \textsf{PTIME} in the size of the game structure and \textsf{EXPTIME} in the size of the acceptance condition~\cite{piterman2006faster}.


\subsubsection{Total-payoff and Mean-payoff Games}

Total-payoff and Mean-payoff games are two-player turn-based games played on edge-weighted graph structure (Figure~\ref{fig:graph-payoff}). The infinite play $\pi$ results in the following payoffs: in Total-payoff games, the reward for player 1 is $\lim\inf_{n\to\infty}\sum_{i=1}^n\pi[i]$ where $\pi[i]$ denotes the weight of the $i^\text{th}$ transition. In Mean-payoff games, the reward is $\lim_{n\to\infty}\frac{1}{n}\sum_{i=1}^n\pi[i]$. They are zero-sum games, meaning that the first player wants to maximize his payoff, and the second player wants to minimize it.


The decision problems associated with these games (whether the payoff is greater than a given value) are known to be in \textsf{NP}$\cap$\textsf{co-NP}. The authors in~\cite{brihaye2017pseudopolynomial} present a pseudo-polynomial algorithm for the total-payoff game in $O(n^4mW^2)$, where $W$ is the maximal absolute value of the weights.


\begin{figure}[H]
    \centering
    \begin{tikzpicture}[
            ->,
            >=stealth',
            shorten >=1pt,
            auto,
            node distance=2.8cm,
            semithick
        ]

      \node[p1node] (A)                    {$q_a$};
      \node[p2node] (B) [above left of=A] {$q_b$};
      \node[p2node] (D) [above right of=A] {$q_d$};
      \node[p1node] (C) [above right of=B] {$q_c$};
      \node[p2node] (E) [right of=D]       {$q_e$};
    
      \path (A) edge [very thick]             node {1} (B)
                edge              node {2} (C)
            (B) edge [loop above] node {1} (B)
                edge [very thick]             node {3} (C)
            (C) edge              node {2} (D)
                edge [very thick, bend left]  node {-2} (E)
            (D) edge [loop below] node {-1} (D)
                edge              node {-1} (A)
            (E) edge [very thick, bend left]  node {-2} (A);
    \end{tikzpicture}
    \caption{Example of a two-player turn-based weighted graph structure. Lozenge states belong to the first player, and round states belong to the second player. Player one can get a null Mean-payoff by forcing the bold cycle. This strategy would also give him a finite Total-payoff. In state $q_d$ player 2 can get a payoff of $-\infty$ by looping in $q_d$.}
    \label{fig:graph-payoff}
\end{figure}

\subsubsection{Energy Games}

Energy games are two-player turn-based games played on edge-weighted graph structures. The first player, $P_1$, has a car on the graph with an initial energy $e_0$. Whenever the car takes an edge with weight $w$, the energy becomes $e_{i+1} = e_i + w$. The game is lost for $P_1$ if the energy gets negative, $P_1$ wins if the car travels forever. This problem is as hard as the Mean-Payoff games~\cite{chatterjee2014polynomial} and is known to be in \textsf{NP}$\cap$\textsf{co-NP}. Under special weight structures, the problem can be solved in \textsf{PTIME}~\cite{chatterjee2014polynomial}.



\subsubsection{Timed Weighted Games Reachability}

In timed weighted games, a player can stay in a state before taking action. Every time step spent in a state costs a given state weight. The reachability objective in this context is for $P_1$ to reach a target node with the least total payoff possible. In the general case, this type of game is undecidable~\cite{brihaye2005optimal}, but some limited cases are proven to be decidable. For instance, the authors in~\cite{busatto2017optimal} solved the game in $2$\textsf{-EXPTIME} and proved the \textsf{EXPTIME} completeness assuming divergence of the weights (intuitively, taking a circuit gives a weight $w$ s.t $\vert w\vert > \epsilon$ for a fixed $\epsilon$).

\section{Multi-Agent System Verification}\label{sec:sys-verif}

In a security game, the actions and objectives of the attacker and defender can be complex and depend on intermediary states of the game (for instance, if the intrusion is detected, the defender may change his strategy). Furthermore, companies use complex risk analysis tools like EBIOS\footnote{\url{https://www.ssi.gouv.fr/en/digital-risk-management/}}, making it hard to define a simple game with simple objectives to model the attack/defense situation. A solution is to use extended Model-checking capabilities on concurrent game structures.

\subsection{Model-Checking}

The model-checking problem is to verify that a model $M$ verifies a property $\psi$ expressed with some property specifications (see Figure~\ref{fig:m-c}), we denote $M\vDash \psi$ for $M$ satisfies $\psi$. If the property is not verified, the model-checker must output a counterexample.

\begin{figure}[H]
    \centering
    \includegraphics[width=\columnwidth]{figures/model-checking.png}
    \caption{Model-Checking principle}
    \label{fig:m-c}
\end{figure}


\begin{figure}
    \centering
    \begin{forest}
      for tree={
        draw,
        minimum height=1cm,
        anchor=parent,
        align=center,
        child anchor=parent
      },
      [{Get malicious code\\on the user device}, name=AD
        [{Bypass the AppStore}]
        [{Exploit vulnerability in installed app}]
        [{Sell/distribute\\malicious app in\\appstore}, angle below
          [{Create malicious\\app}]
          [{Circumvent app\\review}]
          [{Troll/falsify app\\reputation}]
        ]
      ]
    \end{forest}
    \caption{Example of an attack tree. The leaves are atomic attacks step to achieve the subgoals in the upper level of the tree. The subgoal with an arc means the conjunction of the attack step must be achieved. Otherwise, at least one attack step is enough.}
    \label{fig:at}
\end{figure}

\subsection{System Modeling for System Security}

A common representation for the possible attack scenarios of a system is the Attack Tree (example Figure~\ref{fig:at}). It is possible to display the defenses in the attack tree, giving an Attack Defense Tree~\cite{RDK12}.

The authors of~\cite{kumar2015quantitative} model the behavior of an attack tree with weighted timed automata. By combining the automata, they have a complete model of the tree.

In~\cite{gadyatskaya2016modelling}, the system security is modeled as a two-player turn-base game on a  weighted timed stochastic graph structure. The defender plays first from the initial state, choosing which subset of the available defenses he wishes to activate. There is one state per subset of defense. The attacker plays the rest of the game with a reachability objective: he needs to reach a state where the root of the attack tree is compromised.

\subsection{Property Specifications}

Property specification is the expression of a specification in a given language understandable by the model-checker. We will focus on \textit{temporal logics}~\cite{pnueli1977temporal}, a subclass of \textit{modal logics}, that express boolean properties on predicates with temporal operators. The temporal logics are meant to reason about modalities like \textit{"always", "eventually", "often", "now", "later", "while"}...

The first two logics, called \textit{Linear Temporal Logic} and \textit{Computation Tree Logic}, are used on systems described as a Kripke Structure (i.e. state machines describing the states and transition of the system). Then we will see how they are augmented to express properties with strategies in a game setting on concurrent graph structures.

\subsubsection{Linear-time Temporal Logic (LTL)}

\textit{Linear-time Temporal Logic} (LTL) considers time as a suite of unavoidable events or states on a reactive system described as a Kripke structure $\mathcal{S}=\brac{V,E,\Pi,\pi}$. The structure is a directed graph with vertices $V$ and edges $E\subseteq V\times V$, there is a set of proposition $\Pi$, and the observation function $\pi:V\mapsto 2^\Pi$ gives the set of propositions that are true in each vertex.

\paragraph{Syntax.} The following context-free grammar gives an LTL formula with non-terminal and start symbol $\psi$,
$$\psi \longrightarrow p \vert \neg\psi \vert \psi\lor\psi \vert \nnext\psi \vert \psi\until\psi$$
where any $p\in\Pi$ is a terminal symbol.

The $\land$ operator can be derived from $\neg$ and $\lor$, and for an LTL formula $\psi$, we denote $\eventually\psi = \top\until\psi$ and $\always\psi = \neg\eventually\neg\psi$.

\paragraph{Semantic.} We consider a Kripke structure $\mathcal{S}=\brac{V,E,\Pi,\pi}$ and a starting state $v_0\in V$. A valid  computation $\lambda$ on $\mathcal S$ from $v_0$ is an infinite suite of vertices $\lambda=v_0v_1v_2\dots V^*$ starting from $v_0$ and following the edges of the graph. We denote $\lambda[i]$ the $i$\textsuperscript{th} vertex of $\lambda$, and potentially infinite slices by $\lambda[i:j]$ with $j$ excluded. We recursively define the satisfaction of an LTL formula $\psi$ on $\lambda$, noted $\lambda\vDash\psi$,
\begin{itemize}
    \item For $p\in\Pi$, $\lambda\vDash p$ if $p\in\pi(\lambda[0])$,
    \item $\lambda\vDash \neg\psi$ if $\lambda\nvDash\psi$,
    \item $\lambda\vDash \psi_1\lor\psi_2$ if $\lambda\vDash\psi_1\lor \lambda\vDash\psi_2$,
    \item $\lambda\vDash \nnext\psi$ if $\lambda[1:\infty]\vDash\psi$,
    \item $\lambda\vDash \psi_1\until\psi_2$ if there exists $i\in \mathbb N$ such that $\lambda[i:\infty]\vDash\psi_2$ and for all $j<i$, $\lambda[j:\infty]\vDash\psi_1$.
\end{itemize}

As a result, we can give the following interpretation to the temporal operators $\until,\nnext,\eventually$ and $\always$:
\begin{center}
\begin{tabular}{|c|c|}
  \hline
  symbol & interpretation \\
  \hline
  $\until$ & until\\
  $\nnext$ & next\\
  $\always$ & forever\\
  $\eventually$ & eventually\\
  \hline
\end{tabular}
\end{center}

We say that a Kripke structure $\mathcal S$ satisfies an LTL formula $\psi$  from $v_0$, denoted $\mathcal S, v_0 \vDash \psi$ if every valid \textit{computation} starting from $v_0$ in $\mathcal S$ verifies $\psi$.
Finally, $\mathcal S \vDash \psi$ if for all $v\in V$, $\mathcal S,v \vDash \psi$.

\paragraph{Complexity.} The model-checking of an LTL formula $\psi$ on a structure $\mathcal S$ is \textsf{PSPACE}-complete~\cite{sistla1985complexity}, and~\cite{vardi1986automata} proposed an algorithm that runs in $2^{O(\vert \psi\vert)}O(\vert \mathcal{S}\vert)$.

\subsubsection{Computation Tree Logic (CTL)}

In linear-time logic, we considered time as a suit of events bound to happen. In branching-time logic, the future is not determined at a given point in time. A diversity of possible futures can be represented at each moment as in a tree. The Computation Tree Logic (CTL) is a branching-time logic defined with the same temporal operators as LTL ($\until$, $\nnext$, $\always$, and $\eventually$), and with additional path quantifiers ($\forall$ and $\exists$).

\paragraph{Syntax.}  The following context-free grammar gives a CTL formula with non-terminal and start symbol $\psi$,
$$\psi \longrightarrow p \vert \neg\psi \vert \psi\lor\psi \vert \forall\nnext\psi \vert\exists\nnext\psi \vert \forall\psi\until\psi\vert \exists\psi\until\psi$$
where any $p\in\Pi$ is a terminal symbol.

In CTL, every temporal operator is directly preceded by a path quantifier indicating if the property has to be verified on every possible future ($\forall$), or at least one possible future ($\exists$).

\paragraph{Semantic.} Let $\mathcal{S}=\brac{V,E,\Pi,\pi}$ a Kripke structure and $v\in V$. While LTL was decided on paths, CTL has a value on states:
\begin{itemize}
    \item For $p\int \Pi$, $v \vDash p$ if $p \in \pi(v)$,
    \item $v \vDash \neg\psi$ if $v \nvDash\psi$,
    \item $v \vDash \psi_1\lor\psi_2$ if $v \vDash\psi_1\lor v \vDash\psi_2$,
    \item $v \vDash \forall\nnext\psi$ if for all $v'\in V$ such that $(v,v')\in E$, we have $v'\vDash\psi$,
    \item $v \vDash \exists\nnext\psi$ if there is a $v'\in V$ such that $(v,v')\in E$ and $v'\vDash\psi$,
    \item $v \vDash \psi_1\until\psi_2$ if there exists a path $\lambda$ starting from $v$ and an integer $i\in \mathbb N$ such that $\lambda[i]\vDash\psi_2$ and for all $j<i$, $\lambda[j]\vDash\psi_1$,
    \item $v \vDash \psi_1\until\psi_2$ if for all path $\lambda$ starting from $v$, there exists an integer $i\in \mathbb N$ such that $\lambda[i]\vDash\psi_2$ and for all $j<i$, $\lambda[j]\vDash\psi_1$.
\end{itemize}
Moreover, we say the $\mathcal S\vDash \psi$ if, for all $v\in \mathcal{S}$, we have $v\vDash \psi$.

\paragraph{Complexity.} The model-checking of a CTL formula $\psi$ on a structure $\mathcal S$ can be solved in linear time $O(\vert \mathcal{S}\vert\cdot \vert \psi\vert)$\cite{queille1982specification,clarke1986automatic}.

\subsubsection{CTL\textsuperscript{*}}

An important notion in logic is \textit{expressive power}. A logic $L_1$ is as expressive as a logic $L_2$ if for all formula $\psi_2$ of $L_2$, a formula $\psi_1$ of $L_1$ can be built such that it is verified in exactly the same states as $\psi_2$ in any structure $\mathcal{S}$. It has been shown that LTL is not as expressive as CTL (see Figure~\ref{fig:ltl}), and CTL is not as expressive as LTL (see Figure~\ref{fig:ctl} for the intuition). This justifies the need for a more expressive temporal logic. CTL\textsuperscript{*} is an extension of CTL and LTL that is as expressive as CTL and LTL.

\begin{figure}[H]
    \centering
    \begin{tikzpicture}[
            ->,
            >=stealth',
            shorten >=1pt,
            auto,
            node distance=2cm,
            semithick
        ]

      \node[state, initial above] (A) {$p$};
      \node[state] (B) [right of=A] {$\neg p$};
      \node[state] (C) [right of=B] {$p$};

      \path (A) edge[loop left] (A);
      \path (A) edge (B);
      \path (B) edge (C);
      \path (C) edge[loop right] (C);
    \end{tikzpicture}
    \caption{The intuition that the LTL formula $\eventually\always p$ is equivalent to the CTL formula $\forall\eventually\forall\always p$ is wrong. In this structure, $\eventually\always p$ holds because the computations are of the form $p^*(\neg p)p^*\ \vert\ p^*$. However, $\forall\eventually\forall\always p$ does not hold. Indeed, considering the computation $\lambda = p^*$, there is no $i\in \mathbb N$ s.t. $\lambda[i]\vDash \forall\always p$. It can be proven more generally that the LTL formula $\eventually\always p$ does not have equivalent in CTL.}
    \label{fig:ctl}
\end{figure}


\begin{figure}[H]
    \centering
    \subfloat[\centering]{
    \begin{tikzpicture}[
            ->,
            >=stealth',
            shorten >=1pt,
            auto,
            node distance=2cm,
            semithick
        ]

      \node[state, initial above] (A) {$a$};
      \node[state] (B) [below of=A] {$b$};
      \node[state] (C1) [below left of=B] {$p$};
      \node[state] (C2) [below right of=B] {$\neg p$};

      \path (A) edge (B);
      \path (B) edge (C1);
      \path (B) edge (C2);
      \path (C1) edge[loop below] (C1);
      \path (C2) edge[loop below] (C2);
    \end{tikzpicture}
    \label{fig:ltl1}
    }
    \centering
    \subfloat[\centering]{
    \begin{tikzpicture}[
            ->,
            >=stealth',
            shorten >=1pt,
            auto,
            node distance=2cm,
            semithick
        ]

      \node[state, initial above] (A) {$a$};
      \node[state] (B1) [below right of=A] {$b$};
      \node[state] (B2) [below left of=A] {$b$};
      \node[state] (C1) [below of=B1] {$p$};
      \node[state] (C2) [below of=B2] {$\neg p$};

      \path (A) edge (B1);
      \path (A) edge (B2);
      \path (B1) edge (C1);
      \path (B2) edge (C2);
      \path (C1) edge[loop below] (C1);
      \path (C2) edge[loop below] (C2);
    \end{tikzpicture}
    \label{fig:ltl2}
    }
    \caption{For LTL specifications, the structures~\protect\subref{fig:ltl1} and~\protect\subref{fig:ltl2} are equivalents because they generate indistinguishable computations. But the CTL formula $\exists \nnext (\exists\nnext p \land \exists\nnext \neg p)$ ("there exists a next state where there exists a next state with $p$ and a next state with $\neg p$") is true on~\protect\subref{fig:ltl1} but not on~\protect\subref{fig:ltl2}. As a result, LTL is not as expressive as CTL.}
    \label{fig:ltl}
\end{figure}


\paragraph{Syntax.} The following context-free grammar gives a CTL\textsuperscript{*} formula with non-terminals $\psi_{state}$ and $\psi_{path}$, and the start symbol $\psi_{state}$,
\begin{align*}
    \psi_{state} &\longrightarrow p \vert \neg\psi_{state} \vert \psi_{state}\lor\psi_{state} \vert \forall\psi_{path} \vert\exists\psi_{path}\\
    \psi_{path} &\longrightarrow \psi_{state} \vert \neg\psi_{path} \vert \psi_{path} \lor\psi_{path} \vert \nnext\psi_{path} \vert \psi_{path}\until\psi_{path}
\end{align*}
where any $p\in\Pi$ is a terminal symbol.

In CTL, every temporal operator is directly preceded by a path quantifier, but this is no longer required in CTL\textsuperscript{*}.

\paragraph{Semantic.} The semantic for the state formula is the same as in CTL, and the semantic for the path formula is the same as in LTL. There is only the rule $\psi_{path}\longrightarrow\psi_{state}$ left to deal with. A computation $\lambda$ verifies such a $\psi_{path}$ if and only if $\lambda[0]\vDash \psi_{state}$.

\paragraph{Complexity.} It has been shown that CTL\textsuperscript{*} has the same complexity as the LTL model-checking problem. That is CTL\textsuperscript{*} belongs to \textsf{PSPACE-complete}.

\subsubsection{ATL}

The temporal logics seen in the previous subsections (LTL, CTL, and CTL\textsuperscript{*})were interpreted over Kripke structures, whereas the following logics are multi-agent temporal logics and are interpreted over game structures.

ATL~\cite{alur2002alternating} extends CTL in a way that branches are not quantified only with $\forall$ and $\exists$ but are quantified in a more fine-grained way. First, we will define more formally a \textit{concurrent game structure} $S=\brac{k, Q, \Pi, \pi, d, \delta}$ with:
\begin{itemize}
  \item $k$ the number of players, we write $\Sigma=\{1,\dots, k\}$.
  \item $Q$ a finite set of states.
  \item $\Pi$ a finite set of \textit{propositions/observables} (boolean variables).
  \item $\pi:Q\mapsto 2^\Pi$ the \textit{labeling/observation function} telling the propositions that are true in a state $q\in Q$.
  \item For all $a\in \Sigma$, and $q\in Q$, $d_a(q)\geq 1$ is the number of available moves for $a$ in $q$. Let $D(q) = \{1,\dots, d_1(q)\}\times \dots\times\{1,\dots, d_k(q)\}$ be the \textit{move function} that gives the set of \textit{move vectors} from a state $q$.
  \item For $q\in Q$ and a \textit{move vector} $\langle j_1, \dots,j_k\rangle\in D(q)$, the state $\delta(q,j_1,\dots, j_k)\in Q$ is the resulting state from $q$ when each player $a$ do $j_a$. $\delta$ is the \textit{transition function}.
\end{itemize}

\paragraph{Syntax.} The following context-free grammar gives ATL's syntax
with non-terminal and start symbol $\psi$:
$$\psi\longrightarrow p\vert\neg \psi\vert\psi\lor\psi \vert \strat{A}\nnext \psi \vert\strat{A}\psi\until\psi$$
where $p\in\Pi$, and $A\subseteq\Sigma$.

It is similar to CTL, but the new path quantifier is $\strat{A}$ where $A\subseteq \Sigma$ is a \textit{coalition} of players. It can be interpreted as "exists a strategy for the coalition $A$". While $\forall$ means the propriety stands on all outgoing edges and $\exists$ means the propriety stands for at least one outgoing edge, $\strat{A}$ means the propriety stands for at least one edge among the ones controlled by the coalition $A$. As a result, $A$'s protagonists can collaborate to attain their objectives.

\paragraph{Strategy.} To define the semantic of ATL, we need to introduce a formal definition of a strategy. We call a \textit{strategy} for a player $a$, a function $f_a:Q^+\mapsto\mathbb N$ such that for all $\lambda\in Q^+$ finishing in state $q$, $f_a(\lambda) \in \{1,\dots, d_a(q)\}$. It determines the next move for player $a$ after any finite computation.

For a set of \textit{strategies} $F_A=\{f_a\vert a\in A\}$, we denote $out(q,F_A)$ the set of output \textit{computations} where each player in $A$ follows his \textit{strategy}.

\paragraph{Semantic.} Like for CTL, the ATL's semantic is evaluated on states. Given a state $v\in S$, the satisfaction rules for $v\vDash p\in\Pi$, $v\vDash\neg\psi$, and $v\vDash\psi_1\lor\psi_2$ are the same as in CTL. Then we have,
\begin{itemize}
    \item $v\vDash \strat{A}\nnext\psi$ if there exists a set of strategies $F_A$ for players in $A$ s.t. for all $\lambda \in out(q,F_A), \lambda[1] \vDash\psi$.
    \item $v\vDash \strat{A}\psi_1\until\psi_2$  if there exists a set of strategies $F_A$ for players in $A$ s.t. for all $\lambda\in out(q,F_A)$, there exists $i\in\mathbb N$, s.t. $\lambda[i]\vDash\psi_2$ and for all $j< i, \lambda[j] \vDash\psi_1$.
\end{itemize}

\paragraph{Complexity.} The model-checking problem for ATL is \textsf{PTIME-complete} and~\cite{alur2002alternating} proposed an algorithm to solve it in $O(m \cdot \vert \psi\vert)$, for a formula $\psi$ and a concurrent game structure $\mathcal S$ with $m$ transitions.

\subsubsection{ATL\textsuperscript{*}}

The difference between ATL and ATL\textsuperscript{*} is the same as in CTL and CTL\textsuperscript{*}. It is no longer required to have a path quantifier directly in front of every temporal operator.

\paragraph{Syntax.} An ATL\textsuperscript{*} formula is given by the following context-free grammar with non-terminals $\psi_{state}$ and $\psi_{path}$, and start symbol $\psi_{state}$,

\begin{align*}
  \psi_{state}&\longrightarrow p\vert\neg\psi_{state} \vert\psi_{state}\lor\psi_{state} \vert \strat{A}\psi_{path}\\
  \psi_{path}&\longrightarrow\psi_{state}\vert\neg\psi_{path}\vert \psi_{path}\lor\psi_{path}\vert\nnext\psi_{path}\vert\psi_{path}\until\psi_{path}
\end{align*}
where $p\in\Pi$, and $A\subseteq\Sigma$.

\paragraph{Semantic.} For state formulas, the rules are the same as in ATL. Otherwise, for a path formula, a computation $\lambda$ satisfies:

\begin{itemize}
  \item $\lambda\vDash \psi_{state}$, for a state formula $\psi_{state}$, if $\lambda[0]\vDash\psi_{state}$.
  \item $\lambda \vDash \neg\phi_{path}$ if $\lambda\nvDash\phi_{path}$.
  \item $\lambda \vDash \phi_{path,1}\lor\phi_{path,2}$ if $\lambda\vDash\phi_{path,1} \lor\lambda\vDash\phi_{path,2}$.
  \item $\lambda\vDash\nnext\phi_{path}$ if $\lambda[1,\infty]\vDash\phi$.
  \item $\lambda\vDash\phi_{path,1}\until\phi_{path,2}$ if there exists $i\in \mathbb N$ s.t. $\lambda[i,\infty]\vDash\phi_{path,2}\land\forall j<i,\lambda[j,\infty]\vDash \phi_{path,1}$.
\end{itemize}

\paragraph{Complexity.} The model-checking problem of ATL\textsuperscript{*} is in \textsf{2EXPTIME-complete}, but with a bounded size of formula it is \textsf{PTIME-complete}~\cite{alur2002alternating}.
